Summation-by-parts approximations of the second derivative: Pseudoinverses of singular operators and revisiting the sixth order accurate narrow-stencil operator

We consider finite difference approximations of the second derivative, exemplified in Poisson's equation, the heat equation and the wave equation. The finite difference operators satisfy a summation-by-parts property, which mimics the integration-by-parts. Since the operators approximate the second derivative, they are singular by construction. To impose boundary conditions, these operators are modified using Simultaneous Approximation Terms. This makes the modified matrices non-singular, for most choices of boundary conditions. Recently, inverses of such matrices were derived. However, when considering Neumann boundary conditions on both boundaries, the modified matrix is still singular. For such matrices, we have derived an explicit expression for the Moore-Penrose pseudoinverse, which can be used for solving elliptic problems and some time-dependent problems. The condition for this new pseudoinverse to be valid, is that the modified matrix does not have more than one zero eigenvalue. We have reconstructed the sixth order accurate narrow-stencil operator with a free parameter and show that more than one zero eigenvalue can occur. We have performed a detailed analysis on the free parameter to improve the properties of the second derivative operator. We complement the derivations by numerical experiments to demonstrate the improvements of the new second derivative operator.

==> Sections/SecondZeroEigD1.tex <==
\section{Superlong brainstorming about $D_1$}
\label{2ndZeroEigD1}

\sofia{Update: Note that $A_{wide}=D_1^\trans\PH D_1$ is symmetric and therefore a bit more well-behaved. In this case I find one clear zero eigenvalue for all values of $x_1$, and two possible zero eigenvalues around $x_1=0.69$ ($10^{-8}$ and $10^{-6}$).

\ 

}

\sofia{Something about that $D_1$ can be singular, and consequently, in the wide case, $D_2=D_1^2=\PH^{-1}QD_1=\PH^{-1}(-D_1^\trans \PH+\er\er^\trans-\el\el^\trans)D_1$. That is, $A=D_1^\trans\PH D_1$. If $D_1$ has free parameters (which we know they have) giving them 2 zero eigenvalues, then $A$ will also have at least 2 zero eigenvalues. Even if $A$ fulfills the accuracy demands and the SBP-form.
Then, since possible in wide case, perhaps also in the narrow case.

}
\siyang{I have not been able to tune $D_1$ to have 2 zero eigenvalues.}

\sofia{
No, it is tricky, and I am not 100\% sure any longer either (only numerical unclear indications, no proofs).
}


Below, in Figure~\ref{SpectraD1ord6}, the spectra of $D_1$ is shown. The two eigenvalues with smallest absolute value are marked. Note that they are approximately equally big ($\approx0.01$) and far from zero. This is despite the fact that we know that $D_1$ is singular (multiplying by the constant vector returns almost zero ($\approx10^{-13}$)). Matlab returns $\operatorname{rank}(D1)=12$ for all $x_1$, however, the two smallest eigenvalues (supposedly one zero and one not zero) are not distinguishable. \siyang{eig function in MATLAB seems to produce very inaccurate result for $D_1$. I somewhat missed to notice this when investigating $D_1$ :( This behaviour of eig is a mystery to me.}
\begin{figure}[ht]
\centering
\includegraphics[width=.8\textwidth]{Figures/AbsEigsOfD1n12.eps}
\caption{Spectra of $D_1$ (with $n=12$) as a function of the free parameter $x_1$. The second smallest eigenvalue is marked with red.}
\label{SpectraD1ord6}
\end{figure}
By the way, $x_1=342523/518400\approx0.66$ is what I consider the "standard" choice (I don't remember from where I have it though). \siyang{This is a familiar number. Normally, on the first six grid points the truncation error is $\mathcal{O}(h^3)$. With this particular choice, the truncation error on the sixth grid point is $\mathcal{O}(h^4)$, i.e. the free parameter is used to increase the order of accuracy on one grid points. However, with this choice, $D_1$ is not compatible with $D_2$.}
\sofia{Aha, thanks! True, but I think it is still $\mathcal{O}(h^3)$, only smaller error constant. But something is weird here, because when I do the same, I get better values for 0.67 (max norm) or .7 (L2-norm). Do I have bugs?}

It is easier (better? worse?) to study the spectra of $Q$ instead, since it seems better "conditioned" in some sense, see next page.\newpage
In \cite{ref:STRA94} page 59 I found the 6th order accurate operator $D_1$ (denoted $Q$ in \cite{ref:STRA94}, confusing enough). If I plot the absolute values of the eigenvalues of $Q$ (in our notation) as a function of the free parameter $x_1$ I find two candidates where the second smallest eigenvalue is at least close to zero, see Figure~\ref{SpectraQord6}.
\begin{figure}[ht]
\centering
\includegraphics[width=.8\textwidth]{Figures/AbsEigsOfQn12.eps}
\caption{Spectra of $Q$ (with $n=12$) as a function of the free parameter $x_1$. The second smallest eigenvalue is marked with black.}
\label{SpectraQord6}
\end{figure}
If we zoom in around these candidates and make the y-scale logarithmic, see Figure~\ref{SpectraQord6zoom66} and Figure~\ref{SpectraQord6zoom69}, we see that the second smallest eigenvalue goes down significantly. 
\begin{figure}[ht]
\centering
\includegraphics[width=.7\textwidth]{Figures/AbsEigsOfQn12logzoom66.eps}
\caption{Spectra of $Q$ (with $n=12$) as a function of the free parameter $x_1$. Logarithmic y-scale. Zoom around $x_1\approx0.6637$.}
\label{SpectraQord6zoom66}
\end{figure}
However it is difficult to know if values around $10^{-6}$ should qualify as zero or not.  Note that the smallest eigenvalue (which theoretically is exactly equal to zero) also gets "fuzzier" around $x_1\approx0.6637$ and $x_1\approx0.69$. Even though the matrix is only $13\times13$ ($n=12$) the rounding errors play a role. 
\begin{figure}[ht]
\centering
\includegraphics[width=.95\textwidth]{Figures/AbsEigsOfQn12logzoom69.eps}
\caption{Spectra of $Q$ (with $n=12$) as a function of the free parameter $x_1$. Logarithmic y-scale. Zoom around $x_1\approx0.69$.}
\label{SpectraQord6zoom69}
\end{figure}
Is this {\it possible} second zero eigenvalue only present for $n=12$? No, it seems to be rather consistent, see Figure~\ref{2ndsmallest}.
\begin{figure}[ht]
\centering
\includegraphics[width=.65\textwidth]{Figures/2ndSmallestDifferentN.eps}
\caption{Second smallest eigenvalue of $Q$ as a function of $x_1$.}
\label{2ndsmallest}
\end{figure}
Note that if $n$ is an odd number, the second smallest eigenvalue of $Q$ is very small (maybe even zero?)! {\bf Can this really be true?! That would mean that the operators are useless for odd numbers of grid points?}

Well, all in all, these numerical tests are neither a proof of an extra zero eigenvalue nor a proof that such does not exist.

Now I have also tested $\widetilde{Q}=Q+\el\el^\trans$ which should have full rank.
At first it seems that the possible double singularity for $x_1\approx0.69$ is the only one that remains, see Figure~\ref{2ndsmallestQtilde}.
\begin{figure}[ht]
\centering
\includegraphics[width=.65\textwidth]{Figures/AbsEigsOfQsnok12.eps}
\caption{Second smallest eigenvalue of $\widetilde{Q}$ as a function of $x_1$.}
\label{2ndsmallestQtilde}
\end{figure}
However, if zooming in closer to that value, it instead seems as if the two smallest eigenvalues can indeed be very small, but perhaps not zero.
\begin{figure}[ht]
\centering
\includegraphics[width=.65\textwidth]{Figures/AbsEigsOfQsnok12zoom.eps}
\caption{Second smallest eigenvalue of $\widetilde{Q}$ as a function of $x_1$.}
\label{2ndsmallestQtildeZoom}
\end{figure}
